Victima: Drastically Increasing Address Translation Reach by Leveraging Underutilized Cache Resources

Address translation is a performance bottleneck in data-intensive workloads due to large datasets and irregular access patterns that lead to frequent high-latency page table walks (PTWs). PTWs can be reduced by using (i) large hardware TLBs or (ii) large software-managed TLBs. Unfortunately, both solutions have significant drawbacks: increased access latency, power and area (for hardware TLBs), and costly memory accesses, the need for large contiguous memory blocks, and complex OS modifications (for software-managed TLBs). We present Victima, a new software-transparent mechanism that drastically increases the translation reach of the processor by leveraging the underutilized resources of the cache hierarchy. The key idea of Victima is to repurpose L2 cache blocks to store clusters of TLB entries, thereby providing an additional low-latency and high-capacity component that backs up the last-level TLB and thus reduces PTWs. Victima has two main components. First, a PTW cost predictor (PTW-CP) identifies costly-to-translate addresses based on the frequency and cost of the PTWs they lead to. Second, a TLB-aware cache replacement policy prioritizes keeping TLB entries in the cache hierarchy by considering (i) the translation pressure (e.g., last-level TLB miss rate) and (ii) the reuse characteristics of the TLB entries. Our evaluation results show that in native (virtualized) execution environments Victima improves average end-to-end application performance by 7.4% (28.7%) over the baseline four-level radix-tree-based page table design and by 6.2% (20.1%) over a state-of-the-art software-managed TLB, across 11 diverse data-intensive workloads. Victima (i) is effective in both native and virtualized environments, (ii) is completely transparent to application and system software, and (iii) incurs very small area and power overheads on a modern high-end CPU.

==> 05_implementation.tex <==
\section{\system: Detailed Design}
\label{sec:implementation}

We \konrevc{describe} in detail (i) how the L2 cache is modified to store TLB entries, 
(ii) how \system inserts TLB entries \konrevc{into} the L2 cache, 
(iii) how \konrevc{address} translation flow changes in the presence of \system, 
(iv) how \system operates in virtualized environments and 
(v) how \system maintains TLB entries coherent. 
\konrevc{We use as the reference design point a modern x86-64 system that employs 48-bit virtual addresses (VA) and 52-bit physical adddresses (PA)~\cite{intelx86manual}}.

\subsection{Modifications \konrevc{to the} L2 Cache}
\label{sec:l2-changes}
\konrevc{We minimally modify the L2 cache} to (i) support storing TLB entries and (ii) enable a TLB-aware replacement policy 
that favors keeping TLB entries inside the L2 cache taking into account  address translation pressure (e.g., L2 TLB MPKI) and the reuse characteristics of TLB entries. 

\head{\konrevd{TLB Blocks}}
\konrevd{We introduce a new cache block type to store TLB entries in the data store of the L2 cache, called the TLB block.}
\autoref{fig:layout} shows how the same address maps to (i) a conventional L2 data cache block and 
(ii) an L2 cache block that contains TLB entries for 4KB or 2MB pages. 
\konrevc{Each cache entry can potentially store a data block or a TLB block.}
\konrevc{A conventional data block is (typically)} accessed using the PA while \konrevc{a TLB block is} accessed using the VA. 
\system modifies the cache block metadata layout to enable storing TLB entries. 
{First, an additional bit is needed to distinguish between \konrevd{a data block versus a TLB block}. 
Second, in \konrevd{a} conventional data block, the size of the tag of a 1MB, 16-way associative L2 cache consists of $52-log_2(1024)-log_2(64)=36$ bits. 
However, in a TLB block, the tag consists of \konrevc{only} 23 bits and is computed as $48-log_2(4KB)-log_2(1024)-log_2(8)=23$ bits
which is smaller than the tag needed \konrevd{for a data block}.\footnote{\konrevc{Each 64-byte TLB block can store up to 8 8-byte PTEs. Victima uses the 3 least significant bits of the virtual page number to \konrevd{identify and access} a specific PTE.}} 
We leverage the unused space \konrevc{in TLB blocks} to (i) avoid \konrevc{aliasing} and (ii) store page size information.

\begin{figure}[h!]
    \vspace{-2mm}
    \centering
    \includegraphics[width=\linewidth]{figures/camera_ready/layout_l2.pdf}
    \vspace{-5mm}
    \caption{\konkanelloreve{\konrevc{Conventional data block layout} (top) and \konrevc{conventional} TLB block layout for the same address (bottom).}}
    \label{fig:layout}
    \vspace{-2mm}
\end{figure}

To prevent aliasing between the virtual addresses (VAs) of different processes, 
11 unused bits of the tag are reserved for storing the address-space identifier (ASID) or the virtual-machine identifier (VMID) of each process.
The rest of the bits are used \konrevc{to store} page size information.} 
{Given a 48-bit VA and 52-bit PA, we can spare 11 bits for the ASID/VMID. 
As the VA size becomes larger, e.g., 57 bits, fewer bits can be spared for the ASID/VMID (4 bits in case of 57-bit VA and 52-bit PA). 
However, modern operating systems do \emph{not} use more than 12 ASIDs/core~\cite{linuxasid} in order to avoid expensive lookups in the ASID table. 
Hence, when using 57-bit VAs and 52-bit PAs, even with \konrevc{only} 4 bits \konrevc{left} for the ASID, there is no risk of aliasing.}


\konrevc{For a cache with 64-byte cache lines, it is possible to uniquely tag and avoid aliasing between TLB entries \konrevd{(without increasing the size of the cache's hardware tag entries)} only if
$(PA_{length} > VA_{length}-9)$}.\footnote{\konrevd{If $PA_{length} \leq (VA_{length}-9)$, a single VA can map to different TLB blocks. 
This is because the tag of the TLB block does not fit inside the hardware tag entry of the L2 cache.}}
In cases where this condition is not met, an alternative approach is to reduce the number of \konrevd{TLB entries in the TLB Block}
\konrevc{(e.g., \konreve{by} storing 7 PTEs instead of 8 PTEs)} and use the remaining bits for the tag/ASID/VMID. 
Previous works \konrevc{(e.g.,~\cite{graphfire})} propose such solutions to enable efficient sub-block tagging \konreve{in data caches}.

% \todo[color=darkblue!50]{Rev CQ3 QA5 QE1 QE2}






\head{TLB-aware Cache Replacement Policy}
We extend the conventional state-of-the-art SRRIP cache replacement policy~\cite{srrip} to prioritize storing TLB entries \konrevc{of an application} for longer time periods if the application experiences
high address translation overheads (\konrevc{i.e.,} L2 TLB MPKI greater than 5). Listing~\ref{list:srrip} shows the pseudocode of the block insertion function, replacement candidate function, 
and cache hit function for SRRIP in the baseline system and \system (changes compared to baseline SRRIP are marked in blue). 
Upon insertion of a TLB entry inside the L2 cache \nb{(\texttt{insertBlockInL2(block)} Line 1)}, the re-reference interval (analogous to reuse distance) 
is set to 0 (Line 6), marking the TLB entry as a block with a small reuse distance. This way, TLB entries are unlikely to be evicted soon after their insertion. 
\konrevc{Upon selection of a replacement candidate (\texttt{chooseReplacementCandidate()} Line 10), if the selected replacement candidate is a TLB block (Line 23) and translation 
pressure is high (Line 23), SRRIP makes one more attempt to find a replacement candidate that is \emph{not} a TLB block (Line 23).
If no such candidate is found, the TLB block is evicted from the L2 cache and \konrevd{is dropped (i.e., not written anywhere else)}.}
Upon a cache hit to a TLB entry \nb{(\texttt{updateOnL2CacheHit(index)} Line 28)}, the re-reference interval is reduced by three instead of one (Line 32) to provide higher 
priority to the TLB entry compared to other data blocks (Line 34).

% \begin{listing}
% \begin{lstlisting}[caption={TLB-Aware DRRIP L2 Replacement Policy},label={list:srrip}]
% function *@\textbf{insertBlockL2(block)}@*:
%     *@\textcolor{blue}{\textbf{if(block == TLB and TLB\_MPKI > 5) \\ rrip\_counter[block] = 0}}@*

% function *@\textbf{chooseReplacement()}@*:
%     # Search for an invalid line
%     for i from 0 to m_associativity - 1:
%         if (block[i] == invalid ) return i
%     # Perform SRRIP replacement policy
%     for j from 0 to RRIP_MAX:
%         # Search for a line with RRIP_MAX
%         for i from 1 to #ways:
%             *@\textcolor{blue}{\textit{\# If TLB entry and TLB MPKI > 5,}}@*
%             *@\textcolor{blue}{\textit{\# make one more attempt}}@*
%             *@\textcolor{blue}{\textbf{if(block[i] == TLB \&\& TLB\_MPKI > 5) skip}}@* 
%         # Increment all RRIP counters 
%         for i from 1 to #ways :
%             incrementRRIPcounters()

% function *@\textbf{updateOnL2CacheHit(index)}@*:
%     *@\textcolor{blue}{\textit{\# Assume reuse will be high for TLB entry}}@*
%    *@\textcolor{blue}{\textbf{if(block[index] == TLB \&\& TLB\_MPKI > 5)}}@*
%       rrip_counter[index] -= 3;
%    else
%       rrip_counter[index]--;
% \end{lstlisting}
% \vspace{-3mm}
% \rule{\linewidth}{0.5pt}
% \vspace{-8mm}
% %\label{list:srrip}
% \end{listing}
\setcounter{listing}{0}
\setcounter{lstlisting}{0}

\begin{listing}
\begin{lstlisting}[style=customc]
    function *@\textbf{insertBlockInL2(block)}@*:
        // If inserting a TLB block and TLB pressure is high 
        // set the reference-interval to 0 to provide high priority
        // assuming that reuse in near future will be high
        *@\textcolor{blue}{\textbf{if (block == TLB and TLB\_MPKI > 5)}}@*
            *@\textcolor{blue}{rrip\_counter[block] = 0}@*
        else 
            rrip_counter[block] = RRIP_MAX

    function *@\textbf{chooseReplacementCandidate()}@*:
        // Replace an invalid block if possible
        for i from 0 to m_associativity - 1:
            if (block[i] == invalid ) return i
        // Check the re-reference interval of each block in the set
        for j from 0 to RRIP_MAX:
            // Search for a block with RRIP_MAX
            for i from 1 to #ways:
                chosen_block = chooseBlockWithHighRRIP()
                // If a TLB block is chosen for replacement
                // and translation pressure is high, 
                // make one more attempt and try
                // to evict another block if possible
                *@\textcolor{blue}{\textbf{if (chosen\_block == TLB \&\& TLB\_MPKI > 5) skip}}@* 
            // Increment all RRIP counters 
            for i from 1 to #ways :
                incrementRRIPcounters()

    function *@\textbf{updateOnL2CacheHit(index)}@*:
        // Assume reuse will be high for TLB block
        // and reduce the re-reference interval by 3 instead of 1
        *@\textcolor{blue}{\textbf{if (block[index] == TLB \&\& TLB\_MPKI > 5)}}@*
            *@\textcolor{blue}{\textbf{rrip\_counter[index] -= 3;}}@*
        else
            rrip_counter[index]--;
\end{lstlisting}
\vspace{-2mm}
\caption{TLB-Block-Aware SRRIP~\cite{srrip} L2 Cache Replacement Policy}
\vspace{-2mm}
\label{list:srrip}


\end{listing}

\subsection{\konrevc{Inserting} TLB Blocks \konrevd{into} the L2 Cache}
\label{sec:implementation-alloc-native}
\system allocates a \konrevc{block} of 8 TLB entries (64 bytes) that correspond to 8 contiguous virtual pages inside the L2 cache \konrevc{upon} an L2 TLB miss or an L2 TLB eviction,
if the corresponding page \konrevd{is deemed to} be costly-to-translate in the future. To \konrevd{predict} whether a page \konrevc{will be costly-to-translate}, \system employs a Page Table Walk cost predictor (PTW-CP). 
\nb{\autoref{fig:allocation_native} depicts \system's operations on an L2 TLB miss or eviction. }

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{figures/camera_ready/insertion_native.pdf}
    \vspace{-6mm}
    \caption{Insertion of a \konrevd{TLB block into} the L2 cache upon (i) an L2 TLB miss and (ii) an L2 TLB eviction.}
    \label{fig:allocation_native}
    \vspace{-2mm}
\end{figure}

\head{\konrevc{Inserting a TLB Block into the  L2 Cache upon an L2 TLB Miss}}
When an L2 TLB miss occurs, the MMU consults the PTW-CP to find out if the page \konrevd{is predicted to} be costly-to-translate in the future \nb{(\circled{1} in Fig.~\ref{fig:allocation_native})}. 
If the prediction is positive, the MMU checks if the corresponding TLB block already resides inside the L2 cache \nb{\circled{2}}. 
If it does, no further action is needed. If not, the MMU first waits until the PTW is completed \nb{\circled{3b}}.
When the last level of the PT is fetched, the MMU transforms the cache block that contains the PTEs to a TLB block by updating 
the metadata of the block~\nb{\circled{4}}. The MMU (i) replaces the existing tag with the tag of the virtual page region, (ii) 
sets the TLB bit to mark the cache block as TLB block, and (iii) updates the ASID and the page size information \konrevd{associated with the TLB block}. 
This way, the TLB block containing the \konrevc{consecutive} PTE entries is directly accessible using 
the \konrevc{corresponding} virtual page numbers and the ASID of the application \emph{without} walking the PT. 
Storing \konreve{several (e.g., 8 in our implementation)} TLB entries for \konrevd{consecutive} virtual pages inside the \konreve{same} L2 cache \konreve{TLB block} 
can be highly beneficial for applications whose memory acccesses exhibit high spatial locality and frequently access neighboring pages.

\head{\konrevc{Inserting a TLB Block into the L2 Cache upon an L2 TLB Eviction}}
When an L2 TLB eviction occurs, the MMU consults the PTW-CP to find out if the page \konrevd{is predicted to} be costly-to-translate in the future~\nb{(\circled{1} in Fig.~\ref{fig:allocation_native})}. 
If the outcome of the prediction is positive, the MMU checks if the corresponding TLB block already resides in the L2 cache~\nb{\circled{2}}. 
If it does, no further action is needed. If it does not, the MMU issues in the background a PTW for the corresponding TLB entry~\nb{\circled{3a}}. 
When the last level of the page table is fetched~\nb{\circled{3b}}, the MMU follows the same procedure as the L2 TLB miss-based insertion \konrevd{(i.e., transforms the cache block that contains the PTEs to a TLB block)}~\circled{4}.
This way, if the evicted TLB entr\konreva{y} (or any other TLB entry in the block) \konreva{is} accessed again in the future, 
\system can directly access the corresponding PTE without walking the PT. 



\head{Page Table Walk Cost Predictor: Functionality}
The PTW cost predictor (PTW-CP) is a \konrevc{small} \konrevc{comparator-based circuit that} estimates whether the page is among the top 30\% most costly-to-translate pages. \konrevc{Using it,} 
\system \konrevd{predicts} if \konrevc{a} page will cause costly PTWs in the future and decides whether the MMU should store the corresponding TLB block inside the L2 cache.
To make this decision, PTW-CP uses two metrics~\konrevc{associated with a page}: (i) PTW frequency and (ii) PTW cost, \konrevd{both of} which are embedded inside the PTE of the corresponding page. 
Figure~\ref{fig:ptwcp} shows the structure and the functionality of PTW-CP.
PTW frequency is stored as a 3-bit counter in the unused bits of \konrevc{the} PTE and is incremented after every PTW that fetches the corresponding PTE. 
PTW cost is also stored \konrevc{as a 4-bit counter} in the unused bits of the PTE and is incremented every time the PTW \konrevc{leads} to at least one DRAM access.
\konreve{Both counters are updated \konrevd{by the MMU} \konrevc{after} every PTW that fetches the corresponding PTE.}
\konreve{If any of the two counters overflows, its value remains at the maximum value throughout the rest of the program's execution.}


\begin{figure}[h!]
    \vspace{-2mm}
    \centering
    \includegraphics[width=\linewidth]{figures/camera_ready/ptwcp.pdf}
    \vspace{-7mm}
    \caption{Page Table Walk Cost Predictor.}
    \label{fig:ptwcp}
    \vspace{-2mm}
\end{figure}


On an L2 TLB miss or eviction~\circled{1}, the PTW-CP waits until the corresponding PTE is fetched inside the L2 TLB. 
PTW-CP fetches the two counters~\circled{2} from the TLB entry that contains the PTE, passes them through a tree of comparators, and calculates the result~\circled{3}.
If the L2 cache experiences high MPKI \konrevd{(i.e., data exhibits low locality, meaning that caching data is not that beneficial)}, 
the PTW-CP is bypassed and the TLB entry is inserted inside the L2 cache without consulting the PTW-CP~\circled{4}.


\head{Page Table Walk Cost Predictor: Feature Selection}
Our development of PTW-CP's architecture involves a systematic and empirical approach to (i) identify the most critical features for making high-accuracy predictions and
(ii) create an effective predictor while minimizing hardware overhead and inference latency.
Initially, we collect a set of 10 per-page features related to address translation, as shown in Table~\ref{tab:features}.
\konrevd{From} these 10 features, we \konrevd{methodically} identify a \konrevd{small} subset that would maximize accuracy while minimizing \konrevd{prediction} time and storage overhead.


% To ensure a fair comparison, all networks were trained using the Adam optimizer \cite{adam} with a learning rate of $1e^{-3}$ and a cosine learning rate scheduler. The number of layers and the size of hidden layers were optimized using Bayesian Optimization \cite{bo} to achieve the best performance.}

\begin{table}[!ht]
    \centering
    \scriptsize
    \caption{\konkanelloreve{Per-Page Feature Set}}
    \vspace{-4mm}
    \begin{tabular}{|m{12.5em}|m{1em}m{20.5em}|}
    \hline
        \textbf{Feature (per PTE)} & \textbf{Bits} & \textbf{Description} \\ \hline
        Page Size & 1 & The size of the page (4KB or 2MB) \\ 
        \textbf{Page Table Walk Frequency} & \textbf{3} & \textbf{\# of PTWs for the page} \\ 
        \textbf{Page Table Walk Cost} & \textbf{4} & \textbf{\# of DRAM accesses during all PTWs}\\ 
        PWC Hits & 5 & \# of times the PTW led to PWC hit \\ 
        L1 TLB Misses & 5 & \# of times the page experienced L1 TLB miss \\ 
        L2 TLB Misses & 5 & \# of times the page experienced L2 TLB miss \\ 
        L2 Cache Hits & 5 & \# of times the page experienced L2 cache hits \\ 
        L1 TLB Evictions & 5 & \# of times the TLB entry got evicted from L1 TLB \\ 
        L2 TLB Evictions & 6 & \# of times the TLB entry got evicted from L2 TLB \\ 
        Accesses & 6 & \# of accesses to the page \\ \hline
    \end{tabular}
    \label{tab:features}
    \vspace{-1mm}

\end{table}

\konrevd{Table \ref{tab:ptw_perf} shows the architectural characteristics and the performance of three different multi-layer perceptron-based neural networks (NN)~\cite{haykin1994neural} and of \konreve{our} final comparator-based model.}
First, we evaluate three different NN architectures with different feature sets to gain insights about the most critical features (\konrevd{for accuracy}).
The first NN (\texttt{NN-10}) uses all 10 features, the second NN (\texttt{NN-5}) uses a set of 5 features (PTW cost, PTW frequency, PWC hits, L2 TLB evictions, and accesses to the page), 
and the third (\texttt{NN-2}) uses only 2 features, the PTW frequency and the PTW cost.
We use four metrics to evaluate the performance of each model: accuracy, precision, recall, and F1-score.
Accuracy \konrevd{is the fraction} of correct predictions, precision \konrevd{is the fraction} of correct positive \konrevd{(i.e., costly-to-translate)} predictions, 
and recall \konrevd{is the fraction} of correct negative predictions. F1-score is the harmonic mean of precision and recall.
In the context of PTW-CP, making negative predictions when the page is \konrevd{actually} costly-to-translate leads to performance degradation, 
while making positive predictions when the page is \konrevd{actually} \emph{not} costly-to-translate leads to L2 cache pollution.
From Table~\ref{tab:ptw_perf}, we observe that NN-10 achieves the highest performance, with an F1-score of 90.42\%. By reducing the number of features to 5, 
NN-5 still achieves high performance reaching 89.89\% F1-score while NN-2 leads to an F1-score of 80.66\%. 
At the same time, NN-2 is 7.75x smaller than NN-10 and 90.5x smaller than NN-5 which makes it an attractive solution for PTW-CP
as it achieves \konrevd{reasonable} accuracy with \konrevd{small} hardware overhead.




%\begin{figure}[h!]
%    \includegraphics[width=\linewidth]{example-image-duck}
%    \caption{\konkanello{Accuracy/Precision/Recall/F1 score of different networks}}
%\end{figure}
\begin{table}[!ht]
        \centering
    \scriptsize
    \caption{\konkanelloreve{Comparison of Different Types of PTW-CP}}
    \vspace{-4mm}
    \begin{tabular}{|m{12em}|m{4em}m{4em}m{4em}m{7em}|}
    \hline
        \textbf{\textit{Model Parameters}} & \texttt{NN-10} & \texttt{NN-5} & \texttt{NN-2} & \textbf{Comparator} \\ \hline
        \# of Features & 10 & 5 & 2 &\textbf{2} \\ 
        Number of Layers & 4 & 4 & 6 & \textbf{N/A} \\ 
        Size of Hidden Layers & 16 & 64 & 4 & \textbf{N/A} \\ 
        Size (B) & 6024 & 70152 & 776 & \textbf{24} \\ 
        Recall & 93.34\% & 92.44\% & 89.62\% & \textbf{89.61\%} \\ 
        Accuracy & 92.13\% & 91.72\% & 82.90\% & \textbf{82.90\%} \\ 
        Precision & 87.68\% & 87.47\% & 73.33\% & \textbf{73.34\%} \\ 
        F1-score & 90.42\% & 89.89\% & 80.66\% & \textbf{80.66\%} \\ \hline
    \end{tabular}
    \label{tab:ptw_perf}
\end{table}


\konrevc{To gain a better understanding of the prediction pattern of NN-2, Fig.~\ref{fig:scatter} shows the predictions of the network for all possible PTW frequency and PTW cost value pairs. 
We observe that the network exhibits a clear prediction pattern that separates costly-to-translate pages from non-costly-to-translate pages: 
PTW frequency-cost value pairs that fall inside the boundaries of the bounding box (rectangle spanning from the bottom-left corner (1,1) to the top-right corner (12,7) as drawn on Fig.~\ref{fig:scatter}) 
are classified as costly-to-translate by NN-2, while PTW frequency-cost value pairs that fall outside the bounding box are classified as non-costly-to-translate. \konreve{Many of the PTW frequency-cost value pairs
never occur during the execution of the applications we evaluate and are not classified by NN-2.}
Table~\ref{tab:ptw_perf} demonstrates that a simple comparator approach that mimics the functionality the bounding box shown in Fig.~\ref{fig:scatter}, 
achieves an F1-score of 80.66\% without any performance loss compared to NN-2. The comparator-based model requires only 24 bytes of storage,
251x less than NN-10, 2923x less than NN-5 and 32x less than NN-2. The comparator-based model requires only 
(i) four comparators to compare the two counters with the edges of the bounding box, i.e., (1,1) and (12,7)} and (ii) can make a prediction in a single cycle.
The comparator-based model is the PTW-CP architecture that we use in \system.

% \todo[color=darkblue!50]{Rev QE3} 
% \hong{Overall, the systematic and empirical approach undertaken in the development of PTW-CP's architecture allowed for the identification of critical features and the creation of an effective predictor while minimizing overhead and maintaining high performance. The final comparator-based model, based on the insights gained from the neural network approaches, proved to be an efficient solution for PTW-CP.}


%\begin{figure}[h!]
%    \caption{\konkanello{Table with network architectures and features}}
%    \includegraphics[width=\linewidth]{example-image-duck}
%\end{figure}

\begin{figure}[h!]
    \vspace{-2mm}
    \centering
    \includegraphics[width=\linewidth]{figures/camera_ready/ptwcp_bound.pdf}
    \vspace{-6mm}
    \caption{\konkanelloreve{Prediction pattern of NN-2. The bounding box separates the PTW cost-frequency pairs that lead to 
    positive predictions (inside the box) from the ones that lead to negative predictions (outside the box).}}
    \label{fig:scatter}
    \vspace{-4mm}
\end{figure}


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{figures/allocation.pdf}
%     \caption{Allocating TLB entries inside the L2 cache}
%     \label{fig:allocation}
% \end{figure}


\subsection{Address Translation Flow with \system}

\autoref{fig:translation_native} demonstrates the address translation flow in a system that employs \system. 
When \konrevd{an} L2 TLB miss occurs, the MMU in parallel (i) initiates the PTW~\circled{1} and (ii) \konrevd{looks up} \nb{the corresponding TLB block in} the L2 cache~\nb{\circled{2}}.
In contrast \nb{to} regular L2 data block lookups, which are performed using the physical address, a TLB block lookup is performed using the virtual page number (VPN) and the address-space identifier (ASID) of the translation request.
The size of the VPN is not known a priori, so \system probes the L2 cache twice in parallel, once assuming a 4KB VPN and once assuming a 2MB VPN.
If the tag (either the tag of \konrevd{the} 4KB VPN or the tag of the 2MB VPN) and the ASID matches with a block that has the TLB-entry bit set, 
the translation request is served by the L2 cache~\nb{\circled{3a}}, the PTW is aborted, and the TLB entry is inserted into the L2 TLB.
\konrevd{If} the TLB entry is not found in the L2 cache, the PT walker \konrevd{runs to completion and} resolves the translation~\nb{\circled{3b}}.

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{figures/camera_ready/flow_native.pdf}
    \vspace{-5mm}
    \caption{Address translation flow in a system with Victima.}
    \label{fig:translation_native}
    \vspace{-2mm}
\end{figure}
%Whenever an entry is evicted from the L2 TLB, \system uses a PTW cost estimator predictor (\autoref{fig:victima_flow} \circled{5}) 
% to quantify the expected cost of losing this translation: if the cost is deemed to be high, then the evicted translation is inserted into the L2 cache \circled{6} \dbbc{TODO - need to explain what replacement policy: do we evict data blocks or only MD blocks?}.
% \autoref{sec:ptw_cost_estimator} gives more details on the PTW cost estimator.



\subsection{\system in Virtualized Environments}

\konrevd{We} demonstrate how \system improves address translation in virtualized environments. 
The key idea is to insert both (i) TLB entries and (ii) \emph{nested} TLB entries into the L2 cache to 
increase the translation reach of the processor's TLB hierarchy for both guest-virtual-to-guest-physical and 
guest-physical-to-host-physical \konrevd{address} translations and avoid both (i) guest-PTWs and (ii) host-PTWs. 
A nested TLB block is a block of 8 nested TLB entries that correspond to 8 contiguous host-virtual pages. 
\konreve{To distinguish between conventional TLB blocks and nested TLB blocks, \system extends the cache block metadata with an additional bit to mark a block as a nested TLB block.}
\autoref{fig:victima_virt} shows how Nested TLB blocks are inserted into the L2 cache in a system that employs \system and nested paging~\cite{amdnested} in virtualized execution. 
(conventional TLB blocks are allocated as described in \S\ref{sec:implementation-alloc-native}).

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{figures/camera_ready/insertion_virt.pdf}
    \vspace{-4mm}
    \caption{Insertion of a nested TLB block into the L2 cache upon (i)
    a nested TLB miss and (ii) a nested TLB eviction}
    \label{fig:victima_virt}
    \vspace{-2mm}
\end{figure}

\head{\konrevd{Inserting a Nested TLB Block into the L2 Cache upon a Nested TLB Miss}}
\konrevd{When a \konrevd{Nested} TLB miss occurs, the MMU consults the PTW-CP to find out if the host-virtual page will be costly-to-translate in the future \nb{\circled{1}}. 
If the prediction is positive, the MMU checks if the corresponding nested TLB block already resides inside the L2 cache \nb{\circled{2}}. 
If it does, no further action is needed. If not, the MMU first waits until the host-PTW is completed.
When the last level of the host-PT is fetched  \nb{\circled{3b}}, the MMU transforms the cache block that contains the host-PTEs to a nested TLB block by updating 
the metadata of the block~\nb{\circled{4}}. The MMU (i) replaces the existing tag with the tag of the host-virtual page region, (ii) 
sets the nested TLB bit to mark the cache block as a nested TLB block, and (iii) updates the ASID (or VMID) and the page size information.}

\head{\konrevd{Inserting a Nested TLB Block into the L2 Cache upon a Nested TLB Eviction}}
\konrevd{When a \konrevd{Nested} TLB eviction occurs, the MMU consults the PTW-CP to find out if the host-virtual page will be costly-to-translate in the future~\nb{\circled{1}}}. 
If the outcome of the prediction is positive, the MMU checks if the corresponding nested TLB block already resides in the L2 cache~\nb{\circled{2}}. 
If it does, no further action is needed. If it does not, the MMU issues in the background a host-PTW for the corresponding TLB entry~\nb{\circled{3a}}. 
When the last level of the host-PT is fetched~{\circled{3b}}, the MMU transforms the cache block that contains the host-PTEs to a nested TLB block.
~\nb{\circled{4}}.



\head{Address Translation Flow}
\nb{\autoref{fig:victima_virt} shows the address translation flow of a system that employs \system and nested paging~\cite{amdnested} in virtualized execution. }
If a nested TLB miss occurs \nb{\circled{1}}, the MMU probes the L2 cache to search for the nested TLB entry \nb{\circled{2}}. 
If the nested TLB entry is found inside the L2 cache, the host-PTW gets skipped~\nb{\circled{3a}}. 
If it is not found, the host-PTW is performs the guest-physical-to-host-physical address translation \nb{\circled{3b}}.


\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{figures/camera_ready/transflow_virt.pdf}
    \vspace{-6mm}
    \caption{Address translation flow in a system with Victima in a virtualized execution environment.}
    \vspace{-4mm}
\end{figure}

% \subsection{Workloads with High Cache Reuse}
% \konkanellorevb{
% Some data-intensive workloads might experience high locality in the L2 cache. Address translation is usually not a bottleneck in these applications, thus the performance opportunity in speeding up the translations is anyhow low. However, Victima may lead to high cache interference. In applications with high L2 cache reuse, as shown in Listing 1 (Lines 2,14,21) the TLB-aware replacement policy and (PTW-CP) will not advise in favor of storing TLB entries in the L2 cache. To validate our claim, we evaluate 10 Parsec benchmarks~\cite{PARSEC} in a system with Victima and we observe that throughout program execution, only 1\% of the total number of L2 blocks store TLB entries. Hence, we conclude that Victima does not create interference when cache reuse is high. 
% }
% \todo[color=cadmiumgreen!50]{Rev QB2}
% \head{Data vs. TLB Cache Blocks}
% While L2 cache blocks storing data (i.e., blocks for which the \emph{TLB Entry} bit is $0$) 
% %(\autoref{fig:layout}) %
% %\dbb{Add ref to \autoref{fig:victima_flow}?}
% participate in the normal cache coherency protocol, like in the baseline system without \system, TLB blocks (for which the \emph{TLB Entry} bit is $1$) need to \revD{be managed according to the explicit TLB shootdown instructions.} %be managed explicitly and support the same TLB maintenance operations that the TLB hierarchy supports.
% Therefore, \system needs a simple way to (i) decouple TLB blocks from coherency operations and (ii) support the TLB \revD{shootdown} operations.
% %
% % \head{Metadata blocks are not coherent}
% Decoupling TLB blocks from coherency operations can be achieved by propagating the \emph{TLB Entry} bit and ignoring all blocks that have that bit set to $1$, as well as not storing the TLB blocks in any coherency-related structures, such as directories.
% Such a solution (i) requires minimal modifications to the L2 cache and (ii)  reduces coherency traffic when the L2 cache stores is heavily occupied by TLB blocks.
\section{TLB Maintainance Operations}
\label{sec:coherence}
\konkanellorevd{Modern ISAs provide specific instructions used by the OS to invalidate TLB entries and maintain correctness \konrevd{in the presence of} 
(i) context switches and (ii) modifications of virtual-to-physical address mappings (called TLB shootdowns) \konrevd{that} occur \konrevd{due to} physical page migration, memory de-allocation  etc.
Different ISAs provide different instructions for TLB invalidations.
For example, the ARM v8 architecture~\cite[D5.10.2]{arm-manual-tlbmaintenance} defines \konrevd{multiple} special instructions to invalidate TLB entries 
\konrevd{with each instruction handling a distinct case (e.g., invalidating a single TLB entry vs invalidating all TLB entries with a specific ASID).}
x86-64 provides a single instruction, \texttt{INVLPG}, which corresponds to invalidating one single TLB entry~\cite{intelx86manual-vol2}.
In Victima, whenever a TLB invalidation is required, the corresponding TLB entries in the L2 cache need to be invalidated.  
In this section, following the example of the ARM specification, which is a superset of other 
specifications \konreve{we know of}, we discuss in detail how Victima supports TLB invalidations \konrevd{due to} context-switches and TLB shootdowns.}

\subsection{Context Switches}
TLB flushing occurs when the OS \konrevd{switches the hardware context} and schedules another process \konrevd{(or thread)} to the core. 
In this case, the OS makes a decision on whether \konrevd{or not} the TLB entries across the TLB hierarchy \konrevd{should} be invalidated, 
which depends on the ASIDs of the current and to-be-executed processes (in practice Linux uses only 12 different ASIDs per core even though the processor can support up to 4096 ASIDs). 
In Victima, if the OS \konrevd{flushes the \konreve{entire} TLB hierarchy}, \konrevd{all the TLB blocks in L2 cache need to be invalidated as well.}
If the OS performs a partial flush based on the ASID, all the TLB blocks in L2 cache with the corresponding ASID need to be evicted. 
In the corner case that Victima uses fewer bits for the ASID, i.e., when L2 cache tag is not large enough to store \konrevd{enough} ASID bits 
\konrevd{to cover} the ASID of the process, all the TLB blocks inside the L2 cache get invalidated during a context switch 
(the L1 and L2 TLB entries can still be invalidated using the ASID). Based on our evaluation setup, for a 2MB L2 cache which is occupied by 50\% by TLB blocks, 
the total time to complete the invalidation procedure is \konrevd{on} the order of 100 ns.  The invalidation procedure happens in parallel with the L2 TLB 
invalidation and is negligible compared to context switch completion times (order of $\mu$s\VMcontextswitch).


\head{(i) \konrevd{Invalidating} all TLB entries} To invalidate all the TLB blocks inside the L2 cache, the L2 TLB first sends an invalidation command to the L2 cache controller. 
The cache controller \konrevd{probes in parallel} all cache banks to invalidate all the TLB blocks of every L2 \konrevd{cache} set. 
For each way, if the TLB entry bit is set, the TLB block is invalidated.

\head{(ii) \konrevd{Invalidating} all TLB entries with a specific ASID} To invalidate all TLB blocks with a specific ASID, 
the L2 TLB first sends an invalidation command to the L2 cache controller with the corresponding ASID. 
For every cache block, if the TLB entry bit is set and the ASID matches the ASID of the invalidation request, the TLB block is invalidated.
If the size of the ASID of the invalidation command is larger (e.g., 4 bits) than the supported ASID (e.g., 3 bits), then all the TLB blocks inside L2 cache are flushed.
\konreve{However, we believe this is an uncommon case, because, e.g., Linux uses only 12 ASIDs/core~\cite{linuxasid}.}



\subsection{TLB Shootdowns}

\konkanellorevd{A TLB shootdown occurs when the CPU needs to invalidate stale TLB entries on local and remote cores. 
\konrevd{It is caused by various} memory \konrevd{management} operations that modify page table entries, such as de-allocating pages (unmap()), 
migrating pages, page permission changes, deduplication,  and memory compaction. As shown in previous works~\cite{latr}, TLB shootdowns take order of $\mu$s time 
to complete \konrevd{due to} expensive inter-processor interrupts (IPIs). In Victima, if the system performs a TLB shootdown, the corresponding TLB blocks need to be 
invalidated in the L2 cache. We explain how for two different TLB shootdown-based invalidations:}

\konkanellorevd{\head{(i) \konrevd{Invalidating a single TLB entry} given VA and ASID} Invalidating a specific TLB entry by VA and ASID 
only requires sending an invalidation command with the VA and the ASID to the L2 cache controller. 
Since each TLB block contains eight contiguous TLB entries, 
invalidating one TLB entry of the TLB block leads to invalidating all eight corresponding TLB entries.}

\konkanellorevd{\head{(ii) \konrevd{Invalidating all TLB entries given a range of VAs}} Invalidating a range of VAs requires
sending multiple invalidation commands with different VAs to the L2 cache controller. The L2 cache controller 
accordingly invalidates all the corresponding TLB blocks.}

% \todo[color=darkmagenta!50]{Rev QD1 CQ3-QE1 }










\section{Area \& Power Overhead}
\label{sec:overheads}
\konrevd{
\system requires \konrevd{three} \konrevd{additions} to an existing high-performance core design: 
(i) \konrevd{two new \emph{TLB Entry} bits in every L2 cache block (one of TLB entries and one for nested TLB entries)} (\S\ref{sec:l2-changes}), 
(ii) the PTW cost estimator (\S\ref{sec:implementation-alloc-native}) and (iii) the necessary logic to perform tag matching \konreve{and} invalidation of TLB blocks using the \emph{TLB Entry} bit, the VPN, and the ASID (\S\ref{sec:coherence}).
Extending each L2 cache block with two \emph{TLB Entry} bits results in a $0.4\%$ storage overhead for caches with $64$B blocks 
(e.g., in total $8$KB for a $2$MB L2 cache). 
PTW-CP requires only (i) 4 comparators to compare the PTE counters with the corresponding thresholds and (ii) 4 registers to store the thresholds.
To support tag matching/invalidation operations for TLB blocks, we extend the tag comparators of the L2 cache with a bitmask to distinguish between tag matching/invalidation for TLB blocks and tag matching/invalidation for conventional data blocks.
Based on our evaluation with McPAT~\cite{mcpat}, all additional logic requires $0.04\%$ area overhead and $0.08\%$ power overhead on top of the high-end Intel Raptor Lake processor~\cite{raptor_lake}.
}


==> README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************

